Adaptive Gradient Methods Converge Faster with Over-Parameterization (but you should do a line-search)

Adaptive gradient methods are typically used for training over-parameterized models. To better understand their behaviour, we study a simplistic setting -- smooth, convex losses with models over-parameterized enough to interpolate the data. In this setting, we prove that AMSGrad with constant step-size and momentum converges to the minimizer at a faster $O(1/T)$ rate. When interpolation is only approximately satisfied, constant step-size AMSGrad converges to a neighbourhood of the solution at the same rate, while AdaGrad is robust to the violation of interpolation. However, even for simple convex problems satisfying interpolation, the empirical performance of both methods heavily depends on the step-size and requires tuning, questioning their adaptivity. We alleviate this problem by automatically determining the step-size using stochastic line-search or Polyak step-sizes. With these techniques, we prove that both AdaGrad and AMSGrad retain their convergence guarantees, without needing to know problem-dependent constants. Empirically, we demonstrate that these techniques improve the convergence and generalization of adaptive gradient methods across tasks, from binary classification with kernel mappings to multi-class classification with deep networks.

==> Adagrad.tex <==
%!TEX root = main.tex
\section{\adagrad/}
\label{sec:adagrad}
For smooth, convex objectives, \citet{levy2018online} showed that \adagrad/ converges at a rate $\bigO(\nicefrac{1}{T} + \nicefrac{\zeta}{\m!\sqrt{T}})$, 
where $\zeta{}^2 = \sup_\x \E_i[\norm{\grad{\x}-\gradi{\x}}\!{}^2]$ is a uniform bound on the variance of the stochastic gradients. In the over-parameterized setting, we show that \adagrad/ achieves the $\bigO(\nicefrac{1}{T})$ rate when interpolation is exactly satisfied and a slower convergence to the solution if interpolation is violated.\footnote{\red{A similar result also appears in the course notes~\citep{orabona2019modern}.}} The proofs for this section are in~\cref{app:adagrad-proofs}.
\begin{restatable}[Constant step-size \adagrad/]{theorem}{restateThmConstantStepSizeAdagrad}
\label{thm:adagrad-constant}
Assuming (i) convexity and (ii) $L_{\max}$-smoothness of each $f_i$, and (iii) bounded iterates,
\adagrad/ with a constant step-size $\eta$ and uniform averaging such that 
$\bar{\x}_T = \frac{1}{T}\sum_{k=1}^{\raisebox{-.5pt}{\tiny $T$}} \xk$, 
converges at a rate
\begin{align*}
	\Expect{f(\bar{\x}_T) - f^*} 
	\leq \frac{\alpha }{T} + \frac{ \sqrt{\alpha} \sigma}{\sqrt{T}},
	\quad \text{where } \alpha = \frac{1}{2}\paren{\frac{D^2}{\eta} + 2 \eta}^{\!2} d L_{\max}.
\end{align*}
\end{restatable}
When interpolation is exactly satisfied, a similar proof technique can be used to show that \adagrad/ incurs only $O(1)$ regret in the online convex optimization setting (\cref{thm:adagrad-regret} in~\cref{app:adagrad-regret}). The above theorem shows that \adagrad/ is robust to the violation of interpolation and converges to the minimizer at the desired rate for \emph{any} reasonable step-size. Although this is a favourable property, the best constant step-size depends on the problem, and as we demonstrate experimentally in~\cref{sec:experiments}, the performance of \adagrad/ depends on correctly tuning this step-size. 

To overcome this limitation, we use a \emph{conservative Lipschitz line-search} that sets the step-size on the fly, improving the empirical performance of \adagrad/ while retaining its favourable convergence guarantees. At each iteration, this line-search selects a step-size $\etak$ that satisfies the property
\begin{align}
\fk(\xk - \etak \nabla \fk(\xk)) \leq \fk(\xk) -  c \, \etak \norm{\nabla \fk(\xk)}^2, \quad \text{and}\,\, \etak \leq \eta_{k-1}.
\label{eq:conservative-lip-linesearch}
\end{align}
The resulting step-size is then used in the standard \adagrad/ update in~\cref{eq:gen-update}. To find an acceptable step, our results use a backtracking line-search, described in~\cref{app:exp-details}. For simplicity, the theoretical results assume access to the largest step-size that satisfies the above condition.\footnote{The difference between the exact and backtracking line-search is minimal, and the bounds are only changed by a constant depending on the backtracking parameter.} Here, $c$ is a hyper-parameter determined theoretically and typically set to $\nicefrac{1}{2}$ in our experiments. The ``conservative'' part of the line-search is the non-increasing constraint on the step-sizes, which is essential for convergence to the minimizer when interpolation is violated. We refer to it as the \emph{Lipschitz line-search} as it is only used to estimate the local Lipschitz constant. Unlike the classical Armijo line-search for preconditioned gradient descent, the line-search in~\cref{eq:conservative-lip-linesearch} is in the gradient direction, even though the update is in the preconditioned direction. The resulting step-size found is guaranteed to be in the range $\left[\nicefrac{2(1-c)}{L_{\max}},\; \eta_{k-1} \right]$~\citep{vaswani2019painless} and allows us to prove the following theorem. 
\begin{restatable}{theorem}{restateThmLinesearchAdagrad}
\label{thm:adagrad-linesearch-conservative}
Under the same assumptions as~\cref{thm:adagrad-constant}, \adagrad/ with a conservative Lipschitz line-search with $c = 1/2$, a step-size upper bound $\eta_{\max}$ and uniform averaging converges at a rate
\aligns{
\Expect{f(\bar{\x}_T) - f^*} \leq \frac{\alpha}{T} + \frac{\sqrt{\alpha}\sigma}{\sqrt{T}},
\quad \text{where } \alpha = \frac{1}{2} \paren{D^2 \max\left\{\frac{1}{\eta_{\max}}, L_{\max}\right\} + 2 \, \eta_{\max}}^{\m!2} d L_{\max}. 
}
\end{restatable}
Intuitively, the Lipschitz line-search enables \adagrad/ to take larger steps at iterates where the underlying function is smoother. \red{It retains the favourable convergence guarantees of constant step-size \adagrad/, while improving its empirical performance (\cref{sec:experiments}).} Moreover, if interpolation is exactly satisfied, we can obtain an $\bigO(\nicefrac{1}{T})$ convergence without the conservative constraint $\etak \leq \eta_{k-1}$ on the step-sizes (\cref{app:adagrad-interpolation}). 

\iffalse % Check again later
% With a heavy heart, I agree and commented this out.
Inspired by the above result, we consider a simple modification to improve the convergence of SGD with SLS~\citep{vaswani2019painless}. We normalize the step-size (similar to \adagrad/-norm~\citep{ward2018adagrad}) and use the conservative Lipschitz line-search: $\xkk = \xk - \nicefrac{\etak}{\!\sqrt{G_k}} \, \grad{\xk}$ where 
$G_k = \sum_{\raisebox{1pt}{\tiny $j{=}0$}}^{\raisebox{-1.5pt}{\tiny $k$}} \Vert \nabla f_{i_j}(\x_j) \Vert{}^2$ 
and $\etak$ is set using the line-search in~\cref{eq:conservative-lip-linesearch}. 
Using the result in~\cref{thm:adagrad-linesearch-conservative},
%for \small $\Ak = \smallGkSqrt I_d$, 
we conclude that these modifications enable SGD with SLS to converge to the minimizer in contrast to its $\sigma^2$-neighbourhood, without an additional memory or computational overhead.  
\fi
% =============== DUMP =================
% In the next section, we will use Armijo SPS to obtain convergence rates for general preconditioners with bounded eigenvalues. 
% \subsection{General preconditioners with bounded eigenvalues}
% \label{sec:general}
% For general adaptive first-order optimizers such as \adam/, \rmsprop/ and second-order methods 
% like subsampled Newton or L-BFGS, the eigenvalues of the corresponding preconditioner 
% are not guaranteed to monotonically increase across iterations. In the following theorem, we show that as long as the eigenvalues remain bounded, using a constant step-size results in an $\bigO\left(\nicefrac{1}{T} + \sigma^2\right)$ rate. 
% The proofs for \cref{thm:adam-constant,thm:general-armijo-sps} can be found in~\cref{app:general-precond-proofs}.
% \begin{restatable}{theorem}{restateThmConstantAdam}
% \label{thm:adam-constant}
% Under the same assumptions as~\cref{thm:adagrad-constant} and assuming (iv) bounded eigenvalues in the $[a_{\min}, a_{\max}]$ interval, \adam/ with no momentum, constant step-size $\eta = \nicefrac{a_{\min}^2}{2 \, L_{\max} \, a_{\max}}$ and uniform averaging converges at a rate, 
% \aligns{
% 	\Expect{f(\bar{\x}_{T}) - f(\xopt)} & \leq \frac{2 \kappa^2 L_{\max} \norm{\x_0 - \xopt}^2}{T} + \sigma^2, 
% 	\quad \text{where} \, \kappa = \frac{a_{\max}}{a_{\min}}.
% }
% \end{restatable}
% The above results show that constant step-size \adam/ can converges to a minimizer in the interpolation setting. 
% This result does not contradict the counterexample of \citet{reddi2019convergence}, showing the non-convergence of \adam/, since the counterexample does not satisfy interpolation. 
% However, it gives a bound on the neighbourhood in the general stochastic setting 
% and shows that under interpolation, \adam/ without momentum indeed converges to the minimizer. 
% The constant step-size used in the above theorem 
% depends on the eigenvalue bounds of the preconditioner and on the smoothness constant. We can use the Armijo SPS to prove a similar bound without knowledge of the smoothness as follows. 
% \begin{restatable}{theorem}{restateThmSPSAdam}
% \label{thm:general-armijo-sps}
% Under the same assumptions as~\cref{thm:adam-constant}, \adam/ with no momentum, Armijo SPS with $c = \kappa = a_{\max}/a_{\min}$ and uniform averaging converges at a rate, 
% \aligns{
% 	\Expect{f(\bar{\x}_{T}) - f(\xopt)} 
% 	&\leq
%     \frac{\norm{\x_0 - \xopt}^2}{T}
%     \max\left\{\frac{a_{\max} }{\eta_{\max}}, 2 \kappa^2 L_{\max} \right\}
%     \,+\, 
%     \max\left\{1, \frac{4 \eta_{\max} L_{\max} \kappa}{a_{\min}}\right\}\sigma^2.
% }
% \end{restatable}
% This result suggests that we can obtain an $\bigO(\nicefrac{1}{T})$ convergence to the neighbourhood 
% without knowledge of $L_{\max}$. 
% A limitation is that the algorithm still requires knowledge of $\kappa$ to set the step-size. 
% Since the preconditioners do not satisfy a monotonicity property like \amsgrad/, 
% such a dependence seems inevitable in the worst case. However, for the diagonal preconditioners we consider, it is easy to compute $\kappa$, which is simply the largest diagonal divided by the smallest. We remark that it is not possible to prove convergence using Armijo SLS with $c = \kappa > 1$ since it requires $c \leq 1$. 


% For Amsgrad/general - Theorem for constant step-size assuming bounded preconditioner (Needs to be done). 
% In the next section, we show that Armijo SPS can be used to attain faster convergence for general adaptive methods in the strongly-convex setting. 
% \subsection{Line-search}
% \subsubsection{Adagrad}
% \label{sec:adaptive-ls-adagrad}% optimal rate in general stochastic setting
% % Theorem for Lipschitz line-search (Section 4.1 / 4.2)
% % Adagrad-norm - modification to SLS/SPS
% \begin{theorem}[Adagrad with Lipschitz Line-Search]
% Assuming that the iterates remain constrained within a ball of radius $D$ of a global minimum, 
% Adagrad with a Lipschitz Line-Search on an average of $L_{\max}$-smooth, convex function and uniform averaging $\bar{x_T} = \frac{1}{T}\sum_{t=1}^T x_t$ converges at a rate
% \begin{align*}
%     \Expect{f(\bar{x}_T) - f(x^*)}
%     \leq
%     \frac{C L_{\max}}{T}
%     +
%     \frac{L_{\max} \sqrt{C \sigma^2}}{\sqrt{T}},
%     &&
%     C = \paren{\frac{1}{\eta_{\min}}D^2 + \eta_{\max}}^2 d,
% \end{align*}
% where $d$ is the dimension and $\sigma^2$ the expected difference between the minimum value of $f$ and $f_i$, $\sigma^2 = \Expect{f^* - f_i^*}$.
% $\eta_{\max}$ is an arbitrary user-selected bound, while $\eta_{\min}$ is lower-bounded by $1/L_{\max}$ (if $c = 1/2$). $\eta_{\max}$ is extremely pessimistic and unlikely to matter in practice, but worst-case bounds are worst-case.
% \end{theorem}
% \subsection{Amsgrad} 
% \label{sec:adaptive-ls-amsgrad}
% % have the monotonicity property that A_{k+1} > A_k
% % Theorem for Armijo line-search (SLS) (Section 3.1 / 4.3)
% % Can obtain the same bound for SPS - only need a bound on \eta_min

% \begin{theorem}[AMSGrad with Armijo Line-Search]
% Assuming that the iterates remain constrained within a ball of radius $D$ of a global minimum, 
% and that the AMSGrad preconditioner has bounded eigenvalues between $a_{\min}$ and $a_{\max}$,
% AMSgrad without momentum and a conservative (non-increasing) Armijo Line-Search on an average of $L_{\max}$-smooth, convex function and uniform averaging $\bar{x_T} = \frac{1}{T}\sum_{t=1}^T x_t$ converges at a rate
% \begin{align*}
%     \Expect{f(\bar{x}_T) - f(x^*)}
%     \leq
%     6 \frac{a_{\max}L_{\max}}{a_{\min}^2}\frac{D^2}{T} 
%     +
%     2\sigma^2,
% \end{align*}
% where $\sigma^2$ the expected difference between the minimum value of $f$ and $f_i$, $\sigma^2 = \Expect{f^* - f_i^*}$. (if $c = 3/4$).
% Note on $a_{\min}, a_{\max}$: If we assume the gradients are bounded, $\norm{\nabla f_i}^2 \leq G^2$, then $a_{\max} \leq G$,
% and for the diagonal version, $a_{\min}$ is larger than the initial gradient and stabilization term $\epsilon$, $a_{\min} \geq \min_j \norm{\nabla_{x_j} f_i(x_1)} + \epsilon$.
% \end{theorem}
% \sharan{I don't think we need the non-decreasing condition. We definitely don't need it for the interpolation case. And using the SPS proof technique, I would think that we don't need it even for the general case.}

% \subsection{Adam and general preconditioners} 
% \label{sec:adaptive-ls-general}
% % no monotonicity property. 
% % Theorem for SPS - improved bounds (Section 3.2) (Needs to be done)
% (Need to use the SPS proof technique, which had an issue but was just fixed. Will update)
% We first analyze the convergence of adaptive gradient methods in the stochastic, smooth and convex setting. We consider three such methods - Adagrad (Section~\cref{sec:adagrad}), AMSgrad or more generally preconditioners with increasing but bounded eigenvalues in Section~\cref{sec:amsgrad} and finally, in Section~\cref{sec:general}, we analyze a larger class of methods such as RMSProp, L-BFGS that have bounded preconditioners, but do not necessarily satisfy a monotonicity property. 
% Theorem~\citep{thm:adagrad-linesearch-conservative} implies that this update results in an $O\left(\frac{1}{T} + \frac{\sigma^2}{\sqrt{T}}\right)$ convergence to the exact minimizer, improving the convergence of SGD with SLS 


==> Amsgrad.tex <==
%!TEX root = main.tex
\section{\amsgrad/ and non-decreasing preconditioners} %with bounded eigenvalues}
\label{sec:amsgrad}
In this section, we consider \amsgrad/ and, more generally, methods with non-decreasing preconditioners satisfying $A_k \m!\succeq\m! A_{k-1}$. As our focus is on the behavior of the algorithm with respect to the overall step-size, we make the simplifying assumption that the effect of the preconditioning is bounded, meaning that the eigenvalues of $\Ak$ lie in the $\left[ a_{\min}, a_{\max}\right]$ range. This is a common assumption made in the analyses of adaptive methods~\citep{reddi2019convergence, alacaoglu2020new} that prove worst-case convergence rates matching those of SGD. For our theoretical results, we consider the variant of \amsgrad/ without bias correction, as its effect is minimal after the first few iterations. The proofs for this section are in~\cref{app:amsgrad-proofs} and~\cref{app:amsgrad-momentum-proofs}. 

The original analysis of \amsgrad/~\citep{reddi2019convergence} uses a decreasing step-size and a decreasing momentum parameter. It shows an $\bigO(\nicefrac{1}{\!\sqrt{T}})$ convergence for \amsgrad/ in both the smooth and non-smooth convex settings. Recently,~\citet{alacaoglu2020new} showed that this analysis is loose and that \amsgrad/ does not require a decreasing momentum parameter to obtain the $\bigO(\nicefrac{1}{\m!\sqrt{T}})$ rate. However, in practice, \amsgrad/ is typically used with both a constant step-size and momentum parameter. Next, we present the convergence result for this commonly-used variant of \amsgrad/.  
\begin{restatable}{theorem}{restateThmConstantAmsgradmom}
\label{thm:amsgrad-constant-mom}
Under the same assumptions as~\cref{thm:adagrad-constant}, 
and assuming (iv) non-decreasing preconditioners 
(v) bounded eigenvalues in the $[a_{\min}, a_{\max}]$ interval, 
where $\kappa = \nicefrac{a_{\max}}{a_{\min}}$, 
\amsgrad/ with $\beta \in [0,1)$, 
constant step-size $\eta = \frac{1-\beta}{1+\beta}\frac{a_{\min}}{2L_{\max}}$ 
and uniform averaging converges at a rate,
\aligns{
	\Expect{f(\bar{\x}_T) - f^*}
	\leq
	\paren{\frac{1+\beta}{1-\beta}}^{\!\!2}
	\frac{2 L_{\max} D^2 d \kappa}{  T}
	+ \sigma^2.
}
\end{restatable}
When $\sigma = 0$, we obtain a $\bigO(\nicefrac{1}{T})$ convergence to the minimizer. However, when interpolation is only approximately satisfied, we obtain convergence to a neighbourhood with its size depending on $\sigma^2$. We observe that the noise $\sigma^2$ is not amplified because of the non-decreasing momentum (or step-size). A similar distinction between the convergence of constant step-size \adam/ (or \amsgrad/) vs. \adagrad/ has also been recently discussed in the non-convex setting~\citep{defossez2020convergence}. Unfortunately, the final bound is minimized by setting $\beta_{1} = 0$ and our theoretical analysis does not show an advantage of using momentum. Note that this is a common drawback in the analyses of heavy-ball momentum for non-quadratic functions in both the stochastic and deterministic settings~\citep{ghadimi2015global, reddi2019convergence, alacaoglu2020new, sebbouh2020convergence}. 

\newcommand{\fB}{f_{\!\scriptscriptstyle B}}
\newcommand{\xoptB}{x_{\m!\scriptscriptstyle B}^*}
\newcommand{\batchvar}{\sigma_b^{\scriptscriptstyle 2}}

Since \amsgrad/ is typically used for optimizing over-parameterized models, the violation $\sigma^2$ is small, even when interpolation is not exactly satisfied. 
Another reason that constant step-size \amsgrad/ is practically useful is 
because of the use of large batch-sizes that result in a smaller effective neighbourhood. 
To get some intuition about the effect of batch-size, 
note that if we use a batch-size of $b$, 
the resulting neighbourhood depends on 
$\batchvar \coloneqq \E_{B; |B| = b} \left[\fB(\xopt) - \fB(\xoptB) \right]$ 
where $\x^*_B$ is the minimizer of a batch $B$ of training examples. 
By convexity, 
$\batchvar \leq \E [\norm{\xopt - \xoptB} \norm{\nabla \fB(\xopt)}]$. 
If we assume that the distance $\norm{\xopt - \xoptB}$ is bounded, 
$\batchvar \propto \E \Vert\nabla \fB(\xopt)\Vert$. 
Since the examples in each batch are sampled with replacement, 
using the bounds in~\citep{lohr2009sampling}, 
$\batchvar \propto \frac{n  - b}{n b} \norm{\nabla f_{i}(\xopt)}$, 
showing that the effective neighbourhood shrinks as the batch-size becomes larger, 
becoming zero for the full-batch variant. 
With over-parameterization and large batch-sizes, 
the effective neighbourhood is small enough for machine learning tasks 
that do not require exact convergence to the solution. 

The constant step-size required for the above result depends on $L_{\max}$, which is typically unknown. Furthermore, using a global bound on $L_{\max}$ usually results in slower convergence since the local Lipschitz constant can vary considerably during the optimization. To overcome these issues, we use a stochastic variant of the \emph{Armijo line-search}. Unlike the Lipschitz line-search whose sole purpose is to estimate the Lipschitz constant, the Armijo line-search selects a suitable step-size in the preconditioned gradient direction, and as we show in~\cref{sec:experiments}, it results in better empirical performance. Similar to the constant step-size, when interpolation is violated, we only obtain convergence to a neighbourhood of the solution. The stochastic Armijo line-search returns the largest step-size $\etak$ satisfying the following conditions at iteration $k$, 
\begin{align}
\fk(\xk - \etak \Ak^{-1} \gradk{\xk}) \leq \fk(\xk) - c \, \etak \indnormsq{\gradk{\xk}}{\Ak^{-1}}, 
\quad \text{and} \,\, 
\etak \leq \eta_{\max}.
\label{eq:armijo-ls}    
\end{align}
The step-size is artificially upper-bounded by $\eta_{\max}$ 
(typically chosen to be a large value). 
The line-search guarantees descent on the current function $\fk$ 
and that $\etak$ lies in the 
$\left[\nicefrac{2 a_{\min} \, (1-c)}{L_{\max}}, \eta_{\max}\right]$ range. 
In the next theorem, we first consider the variant of \amsgrad/ without momentum ($\beta = 0$)
and show that using the Armijo line-search retains the $O(1/T)$ convergence rate 
without the need to know the Lipschitz constant.
\begin{restatable}{theorem}{restateThmLinesearchAmsgrad}
\label{thm:amsgrad-linesearch}
Under the same assumptions as~\cref{thm:adagrad-constant}, \amsgrad/ with zero momentum, Armijo line-search with $c = \nicefrac{3}{4}$, a step-size upper bound $\eta_{\max}$ and uniform averaging converges at a rate,
\aligns{
	\Expect{f(\bar{\x}_T) - f^*} 
	\leq 
	\paren{\frac{3D^2 d\cdot a_{\max}}{2T} + 3\eta_{\max} \sigma^2}
	\max\left\{\frac{1}{\eta_{\max}}, \frac{2L_{\max}}{a_{\min}}\right\}.
}
\end{restatable}
Comparing this rate with that of using constant step-size (\cref{thm:amsgrad-constant-mom}), we observe that the Armijo line-search results in a worse constant in the convergence rate and a larger neighbourhood. These dependencies can be improved by considering a conservative version of the Armijo line-search. However, we experimentally show that the proposed line-search drastically improves the empirical performance of \amsgrad/. We show that a similar bound also holds for \adagrad/ (see~\cref{cor:adagrad-armijo-interpolation} in~\cref{app:adagrad-proofs}). \adagrad/ with an Armijo line-search converges to a neighbourhood in the absence of interpolation (unlike the results in~\ref{sec:adagrad}). Moreover, the above bound depends on $a_{\min}$ which can be $\bigO(\epsilon)$ in the worst-case, resulting in an unsatisfactory worst-case rate of $\bigO(\nicefrac{1}{\epsilon T})$ even in the interpolation setting. However, like \amsgrad/, \adagrad/ with Armijo line-search has excellent empirical performance, implying the need for a different theoretical assumption in the future. 

Before considering techniques to set the step-size for \amsgrad/ including momentum, we present the details of the stochastic Polyak step-size (SPS)~\citet{loizou2020stochastic, berrada2019training} and Armijo SPS, our modification to the adaptive setting. These variants set the step-size as:
\begin{align*}
	\text{SPS:} \, 
	\etak = \min \m!\left\{\frac{\fk(\xk) - \fkopt}{c \normsq{\sgradf{i_k}{\xk}}}, \eta_{\max} \right\}\m!,
	&&
	\text{Armijo SPS:} \, 
	\etak = \min \m!\left\{\frac{\fk(\xk) - \fkopt}{c \normsq{\sgradf{i_k}{\xk}}_{\Ak^{-1}}}, \eta_{\max} \right\}\m!.
\end{align*}
Here, $\fkopt$ is the minimum value for the function $\fk$.The advantage of SPS over a line-search is that it does not require a potentially expensive backtracking procedure to set the step-size. Moreover, it can be shown that this step-size is always larger than the one returned by line-search, which can lead to faster convergence. However, SPS requires knowledge of $\fjopt$ for each function in the finite-sum. This value is difficult to obtain for general functions but is readily available in the interpolation setting for many machine learning applications. Common loss functions are lower-bounded by zero, and the interpolation setting ensures that these lower-bounds are tight. Consequently, using SPS with $\fjopt \m!=\m! 0$ has been shown to yield good performance for over-parameterized problems~\citep{loizou2020stochastic, berrada2019training}. In~\cref{app:amsgrad-proofs}, we show that the Armijo line-search used for the previous results can be replaced by Armijo SPS and result in similar convergence rates. 

For \amsgrad/ with momentum, we propose to use a \emph{conservative} variant of Armijo SPS that sets $\eta_{\max} = \eta_{k-1}$ at iteration $k$ ensuring that $\etak \leq \eta_{k-1}$. This is because using a  potentially increasing step-size sequence along with momentum can make the optimization unstable and result in divergence. Using this step-size, we prove the following result.
\begin{restatable}{theorem}{restateThmSPSAmsgradmom}
\label{thm:amsgrad-sps-mom}
Under the same assumptions of~\cref{thm:adagrad-constant} and assuming (iv) non-decreasing preconditioners (v) bounded eigenvalues in the $[a_{\min}, a_{\max}]$ interval with $\kappa = \nicefrac{a_{\max}}{a_{\min}}$, \amsgrad/ with $\beta \in [0,1)$, conservative Armijo SPS with $c = \nicefrac{1 + \beta}{1 - \beta}$ and uniform averaging converges at a rate,
\aligns{
\Expect{f(\bar{\x}_T) - f^*}
	\leq
	\paren{\frac{1+\beta}{1-\beta}}^{\!\!2}
	\frac{2 L_{\max} D^2 d \kappa}{  T} 
	+ \sigma^2.
}
\end{restatable}
The above result exactly matches the convergence rate in~\cref{thm:amsgrad-constant-mom} but does not require knowledge of the smoothness constant to set the step-size. Moreover, the conservative step-size enables convergence without requiring an artificial upper-bound $\eta_{\max}$ as in~\cref{thm:amsgrad-constant}. We note that a similar convergence rate can be obtained when using a conservative variant of Armijo SLS (~\cref{app:amsgrad-mom-proofs}), although our theoretical techniques only allow for a restricted range of $\beta$. 

When $\Ak = I_d$, the \amsgrad/ update is equivalent to the update for SGD with heavy-ball momentum~\citep{sebbouh2020convergence}. By setting $\Ak = I_d$ in the above result, we recover an $O(1/T + \sigma^2)$ rate for SGD (using SPS to set the step-size) with heavy-ball momentum. In the smooth, convex setting, our rate matches that of~\citep{sebbouh2020convergence}; however, unlike their result, we do not require knowledge of the Lipschitz constant. This result also provides theoretical justification for the heuristic used for incorporating heavy-ball momentum for SLS in~\citep{vaswani2019painless}. 

For a general preconditioner, the \amsgrad/ update in~\cref{eq:gen-update} 
is not equivalent to heavy-ball momentum. With a constant momentum parameter $\gamma \in [0,1)$, the general heavy-ball update~\citep{loizou2017linearly} is given as $\xkk = \xk - \alpha_k \, \smallAkInverse \gradk{\xk} + \gamma \left(\xk - \xkm \right)$ (refer to~\cref{app:amsgrad-momentum-equivalence} for a relation between the two updates). Unlike this update, \amsgrad/ also preconditions the momentum direction $\paren{\xk - \xkm}$. If we consider the zero-momentum variant of  adaptive gradient methods as preconditioned gradient descent, the above update is a more natural way to incorporate momentum. We explore this alternate method and prove the same $O(1/T + \sigma^2)$ convergence rate for constant step-size, conservative Armijo SPS and Armijo SLS techniques in~\cref{app:amsgrad-hb-proofs}. 
In the next section, we use the above techniques 
for training large over-parameterized deep networks. 
%  is to use the above update for preconditioned SGD with heavy-ball momentum.
% In~\cref{app:amsgrad-momentum-equivalence}, 
% we show that the \amsgrad/ update 
% is equivalent to 

% $\xkk = \xk - \etak (1 -  \beta) \smallAkInverse \gradk{\xk} + \beta \, \frac{\etak}{\eta_{k-1}} \, \smallAkInverse \smallAkm (\xk - \xkm)$. 
% This implies that \amsgrad/ . 

